Linking a universal gas density profile to the core-excised X-ray luminosity in galaxy clusters up to z ~ 1.1

We investigate the regularity of galaxy cluster gas density profiles and the link to the relation between core-excised luminosity, LXc, and mass from the Yx proxy, MYx, for 93 SZE-selected objects. The sample spans masses M500=[0.5 - 20] x 10e14 Msun, and lies at redshifts 0.05<z<1.13. Using XMM-Newton observations, we derive an average ICM density profile for the SZE-selected systems and determine its scaling with mass and redshift. This average profile evolves slightly stronger than self-similar (a_z = 2.09+/-0.02), and has significant dependence on mass (a_M = 0.22 +/- 0.01). Deviations from the average scaling with radius indicate different evolution for the core regions and the bulk. We measure the radial variation of the intrinsic scatter, finding a slight evolution with redshift. The average profile of the SZE-selected systems describes that of X-ray-selected systems at low redshift. The scaled core properties are positively skewed at later times, suggesting an increased incidence of centrally peaked objects at lower redshifts. The relation between LXc and MYx has an intrinsic scatter of 13%. Using simulations, we investigate the impact of selection effects, intrinsic scatter, and covariance on this relation. The slope is insensitive to selection and intrinsic scatter between quantities; however, the scatter is very dependent on the covariance between LXc and Yx. Accounting for our use of the Yx proxy to determine the mass, we estimate an upper limit to the intrinsic scatter with respect to the true mass of 22%. We probe the connection between the scatter in density profiles and that in the LXc-M relation. Our results suggest that the ICM bulk evolves approximately self-similarly, with the core regions evolving separately; indicate a variation of the gas content with mass; and show that LXc has a tight relation to the underlying mass.

==> datatable.tex <==
         RXC\,J$2023.0-2056$  & $0.056    $  & $305.7450    $  & $-20.9485    $& $ 1.21^{+0.03}_{-0.03} $& $ 1.03^{+0.02}_{-0.02} $& $ 0.16^{+0.00}_{-0.00} $& $ 0.40^{+0.01}_{-0.01} $ \\
         RXC\,J$2157.4-0747$  & $0.058    $  & $329.3673    $  & $ -7.8046    $& $ 1.29^{+0.03}_{-0.03} $& $ 1.12^{+0.02}_{-0.02} $& $ 0.15^{+0.00}_{-0.00} $& $ 0.37^{+0.01}_{-0.01} $ \\
         RXC\,J$0345.7-4112$  & $0.060    $  & $ 56.4428    $  & $-41.2042    $& $ 0.97^{+0.02}_{-0.02} $& $ 0.82^{+0.02}_{-0.02} $& $ 0.15^{+0.00}_{-0.00} $& $ 0.37^{+0.01}_{-0.01} $ \\
          RXC\,J$0225.1-2928$  & $0.060    $  & $ 36.2877    $  & $-29.4773    $& $ 0.96^{+0.04}_{-0.04} $& $ 0.73^{+0.02}_{-0.02} $& $ 0.12^{+0.00}_{-0.00} $& $ 0.31^{+0.01}_{-0.01} $ \\
          RXC\,J$1236.7-3354$  & $0.080    $  & $189.1712    $  & $-33.9260    $& $ 1.33^{+0.02}_{-0.02} $& $ 1.21^{+0.02}_{-0.02} $& $ 0.24^{+0.00}_{-0.00} $& $ 0.61^{+0.01}_{-0.01} $ \\
          RXC\,J$2129.8-5048$ & $0.080    $  & $322.4271    $  & $-50.8167    $& $ 2.26^{+0.06}_{-0.06} $& $ 2.23^{+0.04}_{-0.04} $& $ 0.41^{+0.01}_{-0.01} $& $ 1.19^{+0.02}_{-0.02} $ \\
               A 2255  & $0.081    $  & $258.2029    $  & $ 64.0636    $& $ 5.00^{+0.21}_{-0.15} $& $ 6.00^{+0.19}_{-0.16} $& $ 1.24^{+0.01}_{-0.01} $& $ 4.78^{+0.10}_{-0.10} $ \\
         RXC\,J$0821.8+0112$  & $0.082    $  & $125.4614    $  & $  1.1967    $& $ 1.31^{+0.03}_{-0.04} $& $ 1.16^{+0.03}_{-0.03} $& $ 0.22^{+0.00}_{-0.00} $& $ 0.54^{+0.01}_{-0.01} $ \\
           A1651  & $0.084    $  & $194.8438    $  & $ -4.1983    $& $ 4.51^{+0.12}_{-0.11} $& $ 5.63^{+0.13}_{-0.13} $& $ 1.48^{+0.01}_{-0.01} $& $ 5.02^{+0.07}_{-0.07} $ \\
               A 1650  & $0.084    $  & $194.6734    $  & $ -1.7622    $& $ 4.21^{+0.05}_{-0.05} $& $ 5.11^{+0.05}_{-0.05} $& $ 1.27^{+0.00}_{-0.00} $& $ 4.25^{+0.03}_{-0.03} $ \\
          RXC\,J$1302.8-0230$  & $0.085    $  & $195.7216    $  & $ -2.5170    $& $ 1.89^{+0.03}_{-0.03} $& $ 1.80^{+0.02}_{-0.02} $& $ 0.31^{+0.00}_{-0.00} $& $ 0.83^{+0.01}_{-0.01} $ \\
          RXC\,J$0003.8+0203$  & $0.092    $  & $  0.9572    $  & $  2.0657    $& $ 2.11^{+0.04}_{-0.04} $& $ 1.99^{+0.04}_{-0.04} $& $ 0.40^{+0.00}_{-0.00} $& $ 1.15^{+0.01}_{-0.01} $ \\
               A 3921  & $0.094    $  & $342.4917    $  & $-64.4294    $& $ 3.73^{+0.06}_{-0.06} $& $ 4.19^{+0.07}_{-0.06} $& $ 1.07^{+0.00}_{-0.00} $& $ 3.51^{+0.03}_{-0.03} $ \\
           A 3911  & $0.097    $  & $341.5711    $  & $-52.7261    $& $ 3.99^{+0.08}_{-0.08} $& $ 4.87^{+0.09}_{-0.09} $& $ 1.21^{+0.01}_{-0.01} $& $ 3.95^{+0.04}_{-0.04} $ \\
         RXC\,J$2319.6-7313$  & $0.098    $  & $349.9167    $  & $-73.2277    $& $ 1.56^{+0.03}_{-0.03} $& $ 1.74^{+0.03}_{-0.03} $& $ 0.38^{+0.01}_{-0.01} $& $ 0.97^{+0.02}_{-0.01} $ \\
           A 3827  & $0.099    $  & $330.4720    $  & $-59.9454    $& $ 5.64^{+0.09}_{-0.09} $& $ 7.04^{+0.09}_{-0.09} $& $ 1.76^{+0.01}_{-0.01} $& $ 6.61^{+0.06}_{-0.06} $ \\
          RXC\,J$0211.4-4017$  & $0.101    $  & $ 32.8528    $  & $-40.2915    $& $ 1.00^{+0.02}_{-0.02} $& $ 0.98^{+0.01}_{-0.01} $& $ 0.20^{+0.00}_{-0.00} $& $ 0.48^{+0.01}_{-0.00} $ \\
          RXC\,J$0049.4-2931$  & $0.108    $  & $ 12.3460    $  & $-29.5206    $& $ 1.62^{+0.04}_{-0.04} $& $ 1.66^{+0.03}_{-0.03} $& $ 0.38^{+0.01}_{-0.01} $& $ 1.00^{+0.02}_{-0.02} $ \\
               A 2034  & $0.113    $  & $227.5528    $  & $ 33.5104    $& $ 5.64^{+0.14}_{-0.14} $& $ 7.01^{+0.13}_{-0.13} $& $ 1.71^{+0.01}_{-0.01} $& $ 6.34^{+0.10}_{-0.10} $ \\
          RXC\,J$0006.0-3443$  & $0.115    $  & $  1.5015    $  & $-34.7224    $& $ 3.95^{+0.12}_{-0.12} $& $ 4.48^{+0.11}_{-0.11} $& $ 0.97^{+0.01}_{-0.01} $& $ 3.17^{+0.05}_{-0.05} $ \\
         RXC\,J$0616.8-4748$  & $0.116    $  & $ 94.2158    $  & $-47.7950    $& $ 2.70^{+0.05}_{-0.05} $& $ 2.86^{+0.04}_{-0.04} $& $ 0.60^{+0.01}_{-0.01} $& $ 1.88^{+0.02}_{-0.02} $ \\
          RXC\,J$0145.0-5300$  & $0.117    $  & $ 26.2433    $  & $-53.0208    $& $ 4.37^{+0.08}_{-0.08} $& $ 4.85^{+0.06}_{-0.06} $& $ 1.08^{+0.01}_{-0.01} $& $ 3.87^{+0.03}_{-0.03} $ \\
          RXC\,J$1516.3+0005$  & $0.118    $  & $229.0747    $  & $  0.0893    $& $ 3.28^{+0.07}_{-0.04} $& $ 3.61^{+0.04}_{-0.03} $& $ 0.89^{+0.01}_{-0.01} $& $ 2.76^{+0.02}_{-0.02} $ \\
          RXC\,J$2149.1-3041$  & $0.118    $  & $327.2817    $  & $-30.7013    $& $ 2.25^{+0.03}_{-0.03} $& $ 2.48^{+0.03}_{-0.03} $& $ 0.55^{+0.00}_{-0.00} $& $ 1.58^{+0.02}_{-0.01} $ \\
          RXC\,J$1141.4-1216$  & $0.119    $  & $175.3513    $  & $-12.2776    $& $ 2.27^{+0.02}_{-0.02} $& $ 2.45^{+0.02}_{-0.02} $& $ 0.60^{+0.00}_{-0.00} $& $ 1.69^{+0.01}_{-0.01} $ \\
          RXC\,J$1516.5-0056$  & $0.120    $  & $229.1842    $  & $ -0.9696    $& $ 2.59^{+0.05}_{-0.04} $& $ 2.99^{+0.04}_{-0.04} $& $ 0.62^{+0.01}_{-0.01} $& $ 1.77^{+0.02}_{-0.02} $ \\
          RXC\,J$1044.5-0704$  & $0.134    $  & $161.1370    $  & $ -7.0687    $& $ 2.69^{+0.02}_{-0.02} $& $ 3.32^{+0.04}_{-0.04} $& $ 1.04^{+0.01}_{-0.01} $& $ 2.99^{+0.02}_{-0.02} $ \\
          RXC\,J$0605.8-3518$  & $0.139    $  & $ 91.4752    $  & $-35.3023    $& $ 3.89^{+0.09}_{-0.09} $& $ 4.66^{+0.08}_{-0.08} $& $ 1.27^{+0.01}_{-0.01} $& $ 4.23^{+0.16}_{-0.03} $ \\
%          R0605\_3518  & $0.139    $  & $ 91.4752    $  & $-35.3023    $& $ 3.87^{+0.06}_{-0.06} $& $ 4.63^{+0.05}_{-0.05} $& $ 1.27^{+0.01}_{-0.01} $& $ 4.23^{+0.04}_{-0.03} $ \\
          RXC\,J$0020.7-2542$  & $0.141    $  & $  5.1755    $  & $-25.7080    $& $ 3.84^{+0.06}_{-0.06} $& $ 4.06^{+0.06}_{-0.06} $& $ 1.17^{+0.01}_{-0.01} $& $ 4.05^{+0.04}_{-0.03} $ \\
          RXC\,J$2218.6-3853$  & $0.141    $  & $334.6677    $  & $-38.9018    $& $ 4.92^{+0.11}_{-0.11} $& $ 5.67^{+0.07}_{-0.07} $& $ 1.50^{+0.02}_{-0.02} $& $ 5.56^{+0.06}_{-0.06} $ \\
 %         R2218\_3853  & $0.141    $  & $334.6677    $  & $-38.9018    $& $ 4.92^{+0.14}_{-0.14} $& $ 5.66^{+0.11}_{-0.11} $& $ 1.50^{+0.02}_{-0.02} $& $ 5.56^{+0.07}_{-0.06} $ \\
               A 1413  & $0.143    $  & $178.8250    $  & $ 23.4049    $& $ 6.24^{+0.06}_{-0.06} $& $ 8.13^{+0.06}_{-0.05} $& $ 2.27^{+0.01}_{-0.01} $& $ 8.84^{+0.06}_{-0.06} $ \\
          RXC\,J$2048.1-1750$  & $0.147    $  & $312.0419    $  & $-17.8413    $& $ 4.31^{+0.07}_{-0.07} $& $ 5.50^{+0.05}_{-0.05} $& $ 1.36^{+0.01}_{-0.01} $& $ 4.40^{+0.03}_{-0.03} $ \\
          RXC\,J$0547.6-3152$  & $0.148    $  & $ 86.9081    $  & $-31.8727    $& $ 5.01^{+0.10}_{-0.10} $& $ 5.97^{+0.08}_{-0.07} $& $ 1.58^{+0.01}_{-0.01} $& $ 5.73^{+0.38}_{-0.04} $ \\
%          R0547\_3152  & $0.148    $  & $ 86.9081    $  & $-31.8727    $& $ 4.98^{+0.09}_{-0.08} $& $ 5.94^{+0.05}_{-0.04} $& $ 1.58^{+0.01}_{-0.01} $& $ 5.73^{+0.04}_{-0.04} $ \\
          RXC\,J$2217.7-3543$  & $0.149    $  & $334.4400    $  & $-35.7260    $& $ 3.61^{+0.05}_{-0.05} $& $ 4.37^{+0.04}_{-0.04} $& $ 1.15^{+0.01}_{-0.01} $& $ 3.68^{+0.03}_{-0.03} $ \\
%          R2217\_3543  & $0.149    $  & $334.4400    $  & $-35.7260    $& $ 3.64^{+0.09}_{-0.06} $& $ 4.40^{+0.07}_{-0.06} $& $ 1.15^{+0.01}_{-0.01} $& $ 3.68^{+0.03}_{-0.03} $ \\
         RXC\,J$2234.5-3744$  & $0.151    $  & $338.6125    $  & $-37.7360    $& $ 7.36^{+0.09}_{-0.09} $& $ 9.87^{+0.10}_{-0.11} $& $ 3.05^{+0.02}_{-0.02} $& $12.28^{+0.12}_{-0.10} $ \\
%         R2234\_3744b  & $0.151    $  & $338.6125    $  & $-37.7360    $& $ 7.31^{+0.14}_{-0.14} $& $ 9.72^{+0.17}_{-0.17} $& $ 3.05^{+0.02}_{-0.02} $& $12.28^{+0.12}_{-0.10} $ \\
           A 2204  & $0.152    $  & $248.1959    $  & $  5.5754    $& $ 8.06^{+0.23}_{-0.22} $& $10.94^{+0.26}_{-0.25} $& $ 2.96^{+0.02}_{-0.02} $& $12.51^{+0.17}_{-0.17} $ \\
                A 868  & $0.153    $  & $146.3575    $  & $ -8.6557    $& $ 3.91^{+0.15}_{-0.11} $& $ 5.04^{+0.13}_{-0.10} $& $ 1.43^{+0.02}_{-0.02} $& $ 4.66^{+0.08}_{-0.08} $ \\
          RXC\,J$2014.8-2430$  & $0.154    $  & $303.7154    $  & $-24.5059    $& $ 5.38^{+0.07}_{-0.07} $& $ 7.19^{+0.07}_{-0.07} $& $ 2.08^{+0.02}_{-0.02} $& $ 7.47^{+0.07}_{-0.06} $ \\
      RX\,J1720.1+2638  & $0.164    $  & $260.0417    $  & $ 26.6250    $& $ 5.30^{+0.11}_{-0.11} $& $ 6.97^{+0.12}_{-0.12} $& $ 2.06^{+0.02}_{-0.02} $& $ 7.49^{+0.08}_{-0.08} $ \\
         RXC\,J$0645.4-5413$  & $0.164    $  & $101.3712    $  & $-54.2273    $& $ 7.38^{+0.18}_{-0.18} $& $10.04^{+0.18}_{-0.18} $& $ 2.81^{+0.02}_{-0.02} $& $11.33^{+0.25}_{-0.08} $ \\
%         R0645\_5413c  & $0.164    $  & $101.3712    $  & $-54.2273    $& $ 7.38^{+0.14}_{-0.14} $& $10.08^{+0.11}_{-0.11} $& $ 2.81^{+0.02}_{-0.02} $& $11.33^{+0.10}_{-0.08} $ \\
          RXC\,J$0958.3-1103$  & $0.167    $  & $149.5930    $  & $-11.0644    $& $ 4.17^{+0.22}_{-0.15} $& $ 4.43^{+0.21}_{-0.20} $& $ 1.42^{+0.04}_{-0.04} $& $ 5.21^{+0.15}_{-0.14} $ \\
               A 2218  & $0.171    $  & $248.9597    $  & $ 66.2125    $& $ 5.37^{+0.10}_{-0.10} $& $ 7.41^{+0.10}_{-0.10} $& $ 2.20^{+0.01}_{-0.01} $& $ 7.76^{+0.09}_{-0.09} $ \\
               A 1914  & $0.171    $  & $216.5105    $  & $ 37.8243    $& $ 8.25^{+0.19}_{-0.19} $& $10.80^{+0.19}_{-0.20} $& $ 3.23^{+0.02}_{-0.02} $& $14.34^{+0.18}_{-0.18} $ \\
                A 665  & $0.182    $  & $127.7462    $  & $ 65.8398    $& $ 8.07^{+0.53}_{-0.42} $& $11.27^{+0.55}_{-0.45} $& $ 3.04^{+0.06}_{-0.06} $& $13.15^{+0.41}_{-0.41} $ \\
          RXC\,J$1311.4-0120$  & $0.183    $  & $197.8727    $  & $ -1.3415    $& $ 8.41^{+0.08}_{-0.08} $& $10.69^{+0.06}_{-0.06} $& $ 3.36^{+0.01}_{-0.01} $& $14.93^{+0.08}_{-0.07} $ \\
%           Abell1689  & $0.183    $  & $197.8726    $  & $ -1.3417    $& $ 8.19^{+0.11}_{-0.11} $& $10.79^{+0.10}_{-0.10} $& $ 3.45^{+0.01}_{-0.01} $& $15.24^{+0.12}_{-0.12} $ \\
            A 520  & $0.203    $  & $ 73.5402    $  & $  2.9212    $& $ 8.31^{+0.22}_{-0.21} $& $11.40^{+0.20}_{-0.18} $& $ 3.46^{+0.03}_{-0.03} $& $14.83^{+0.22}_{-0.22} $ \\
               A 2163  & $0.203    $  & $243.9399    $  & $ -6.1491    $& $20.10^{+0.61}_{-0.62} $& $32.27^{+0.68}_{-0.70} $& $ 9.50^{+0.08}_{-0.08} $& $55.06^{+1.00}_{-1.00} $ \\
            A 963  & $0.206    $  & $154.2653    $  & $ 39.0482    $& $ 5.02^{+0.10}_{-0.10} $& $ 6.67^{+0.09}_{-0.09} $& $ 2.15^{+0.02}_{-0.02} $& $ 7.74^{+0.10}_{-0.10} $ \\
            A 773  & $0.217    $  & $139.4765    $  & $ 51.7315    $& $ 6.61^{+0.14}_{-0.14} $& $ 8.86^{+0.11}_{-0.12} $& $ 2.75^{+0.02}_{-0.02} $& $10.85^{+0.12}_{-0.12} $ \\
           A 1763  & $0.223    $  & $203.8298    $  & $ 41.0001    $& $ 7.38^{+0.18}_{-0.18} $& $11.36^{+0.20}_{-0.20} $& $ 3.58^{+0.02}_{-0.02} $& $13.63^{+0.16}_{-0.16} $ \\
           A 2261  & $0.224    $  & $260.6127    $  & $ 32.1324    $& $ 6.33^{+0.59}_{-0.51} $& $ 9.25^{+0.66}_{-0.58} $& $ 3.15^{+0.13}_{-0.13} $& $12.33^{+0.65}_{-0.65} $ \\
               A 2219  & $0.228    $  & $250.0837    $  & $ 46.7107    $& $11.62^{+0.33}_{-0.24} $& $17.60^{+0.31}_{-0.25} $& $ 6.31^{+0.05}_{-0.05} $& $30.96^{+0.54}_{-0.54} $ \\
               A 2390  & $0.231    $  & $328.4031    $  & $ 17.6949    $& $10.67^{+0.28}_{-0.28} $& $15.86^{+0.32}_{-0.31} $& $ 5.61^{+0.05}_{-0.05} $& $25.89^{+0.38}_{-0.38} $ \\
     RXC\,J$0303.8-7752$  & $0.274    $  & $ 45.9366    $  & $-77.8784    $& $ 7.54^{+0.31}_{-0.32} $& $ 9.76^{+0.26}_{-0.28} $& $ 3.16^{+0.04}_{-0.04} $& $13.35^{+0.28}_{-0.28} $ \\
     RXC\,J$0532.9-3701$  & $0.275    $  & $ 83.2323    $  & $-37.0270    $& $ 6.40^{+0.23}_{-0.23} $& $ 8.54^{+0.21}_{-0.22} $& $ 2.96^{+0.04}_{-0.04} $& $11.77^{+0.23}_{-0.23} $ \\
     RXC\,J$0232.2-4420$  & $0.284    $  & $ 38.0772    $  & $-44.3464    $& $ 6.99^{+0.21}_{-0.20} $& $10.81^{+0.23}_{-0.23} $& $ 4.34^{+0.04}_{-0.04} $& $16.28^{+0.27}_{-0.27} $ \\
     RXC\,J$0528.9-3927$  & $0.284    $  & $ 82.2211    $  & $-39.4714    $& $ 6.86^{+0.30}_{-0.33} $& $11.09^{+0.31}_{-0.31} $& $ 4.18^{+0.05}_{-0.05} $& $15.29^{+0.37}_{-0.37} $ \\
     RXC\,J$0043.4-2037$  & $0.292    $  & $ 10.8519    $  & $-20.6229    $& $ 5.91^{+0.25}_{-0.18} $& $ 8.75^{+0.24}_{-0.20} $& $ 3.38^{+0.04}_{-0.04} $& $12.36^{+0.25}_{-0.25} $ \\
     RXC\,J$0516.7-5430$  & $0.295    $  & $ 79.1536    $  & $-54.5090    $& $ 7.81^{+0.81}_{-0.73} $& $11.94^{+0.98}_{-0.96} $& $ 3.90^{+0.17}_{-0.17} $& $15.98^{+0.95}_{-0.95} $ \\
          RXC\,J$0658.4-5557$  & $0.296    $  & $104.6277    $  & $-55.9434    $& $13.92^{+0.29}_{-0.28} $& $20.97^{+0.29}_{-0.28} $& $ 8.72^{+0.06}_{-0.06} $& $46.88^{+0.53}_{-0.53} $ \\
                A 781  & $0.298    $  & $140.1018    $  & $ 30.5028    $& $ 5.36^{+0.09}_{-0.09} $& $ 7.55^{+0.09}_{-0.09} $& $ 2.63^{+0.02}_{-0.02} $& $ 9.46^{+0.11}_{-0.11} $ \\
               A 576  & $0.302    $  & $189.2441    $  & $ 63.1871    $& $ 5.67^{+0.44}_{-0.39} $& $ 7.97^{+0.47}_{-0.43} $& $ 2.99^{+0.09}_{-0.09} $& $11.43^{+0.53}_{-0.53} $ \\
     RXC\,J$0014.3-3022$ & $0.307    $  & $  3.5775    $  & $-30.3863    $& $ 9.81^{+0.24}_{-0.24} $& $16.49^{+0.23}_{-0.22} $& $ 6.70^{+0.05}_{-0.05} $& $27.83^{+0.32}_{-0.32} $ \\
     RXC\,J$1131.9-1955$  & $0.308    $  & $172.9775    $  & $-19.9285    $& $ 8.61^{+0.33}_{-0.30} $& $13.14^{+0.33}_{-0.33} $& $ 4.68^{+0.05}_{-0.05} $& $18.93^{+0.31}_{-0.31} $ \\
     PLCK\,G$103.6+24.8$  & $0.330    $  & $286.1007    $  & $ 72.4622    $& $ 4.89^{+0.24}_{-0.23} $& $ 5.34^{+0.21}_{-0.20} $& $ 1.45^{+0.03}_{-0.03} $& $ 6.09^{+0.15}_{-0.15} $ \\
              AS 1063  & $0.347    $  & $342.1824    $  & $-44.5305    $& $12.66^{+0.27}_{-0.27} $& $19.02^{+0.27}_{-0.26} $& $ 8.49^{+0.06}_{-0.06} $& $44.19^{+0.63}_{-0.63} $ \\
             RX\,J$2228.6+2037$  & $0.412    $  & $337.1405    $  & $ 20.6204    $& $ 8.70^{+0.28}_{-0.28} $& $13.21^{+0.27}_{-0.27} $& $ 5.24^{+0.05}_{-0.05} $& $23.01^{+0.43}_{-0.43} $ \\
             RX\,J$1206.2-0848$  & $0.441    $  & $181.5521    $  & $ -8.8002    $& $10.76^{+0.30}_{-0.30} $& $15.71^{+0.28}_{-0.28} $& $ 6.79^{+0.06}_{-0.06} $& $33.82^{+0.65}_{-0.65} $ \\
    MACS\,J2243.3-0935  & $0.444    $  & $340.8387    $  & $ -9.5947    $& $ 9.10^{+0.12}_{-0.12} $& $14.71^{+0.13}_{-0.13} $& $ 7.30^{+0.03}_{-0.03} $& $31.65^{+0.26}_{-0.26} $ \\
     PLCK\,G$254.1-58.4$  & $0.458    $  & $ 46.0705    $  & $-44.0257    $& $ 5.84^{+0.33}_{-0.33} $& $ 8.21^{+0.33}_{-0.32} $& $ 3.19^{+0.06}_{-0.06} $& $11.74^{+0.32}_{-0.32} $ \\
     RXC\,J$0243.6-4834$  & $0.500    $  & $ 40.9129    $  & $-48.5611    $& $ 6.13^{+0.63}_{-0.45} $& $ 8.11^{+0.52}_{-0.41} $& $ 3.10^{+0.08}_{-0.08} $& $12.46^{+0.57}_{-0.57} $ \\
      PLCK\,G$44.7-51.3$  & $0.503    $  & $333.7383    $  & $-14.0045    $& $ 7.95^{+0.44}_{-0.43} $& $11.64^{+0.46}_{-0.45} $& $ 5.29^{+0.08}_{-0.08} $& $22.64^{+0.66}_{-0.66} $ \\
     PLCK\,G$211.2+38.6$  & $0.505    $  & $137.7970    $  & $ 17.7760    $& $ 5.48^{+0.22}_{-0.22} $& $ 7.35^{+0.21}_{-0.21} $& $ 3.03^{+0.04}_{-0.04} $& $11.51^{+0.26}_{-0.26} $ \\
       PLCK\,G$4.5-19.5$  & $0.516    $  & $289.2692    $  & $-33.5228    $& $ 8.73^{+0.48}_{-0.48} $& $12.58^{+0.53}_{-0.52} $& $ 6.28^{+0.15}_{-0.15} $& $28.93^{+1.05}_{-1.05} $ \\
     PLCK\,G$111.1-87.5$  & $0.520    $  & $ 12.2939    $  & $-24.6792    $& $ 4.83^{+0.46}_{-0.36} $& $ 5.45^{+0.43}_{-0.36} $& $ 2.30^{+0.08}_{-0.08} $& $ 8.25^{+0.38}_{-0.38} $ \\
     PLCK\,G$212.5+63.2$  & $0.529    $  & $163.2159    $  & $ 24.2584    $& $ 4.15^{+0.23}_{-0.23} $& $ 5.35^{+0.21}_{-0.21} $& $ 1.93^{+0.04}_{-0.04} $& $ 7.08^{+0.25}_{-0.25} $ \\
       MS\,$0451.6-0305$  & $0.538    $  & $ 73.5471    $  & $ -3.0162    $& $ 7.90^{+0.30}_{-0.29} $& $11.18^{+0.31}_{-0.29} $& $ 6.47^{+0.07}_{-0.07} $& $28.31^{+0.57}_{-0.57} $ \\
      PLCK\,G$94.6+51.0$ & $0.539    $  & $227.0821    $  & $ 57.9164    $& $ 6.15^{+0.25}_{-0.24} $& $ 8.90^{+0.23}_{-0.22} $& $ 3.87^{+0.05}_{-0.05} $& $14.86^{+0.34}_{-0.34} $ \\
     PLCK\,G$228.2+75.2$  & $0.544    $  & $177.3976    $  & $ 22.4011    $& $ 9.36^{+0.64}_{-0.62} $& $14.77^{+0.77}_{-0.73} $& $ 7.08^{+0.17}_{-0.17} $& $31.46^{+1.15}_{-1.15} $ \\
    MACS\,J$0717.5+3745$  & $0.546    $  & $109.3800    $  & $ 37.7587    $& $12.83^{+0.17}_{-0.17} $& $22.16^{+0.20}_{-0.20} $& $11.41^{+0.04}_{-0.04} $& $56.07^{+0.41}_{-0.41} $ \\
           CL\,0016+16  & $0.546    $  & $  4.6399    $  & $ 16.4362    $& $ 9.21^{+0.24}_{-0.24} $& $14.41^{+0.25}_{-0.25} $& $ 7.49^{+0.07}_{-0.07} $& $34.24^{+0.52}_{-0.52} $ \\
     PLCK\,G$183.9+43.0$  & $0.559    $  & $137.7032    $  & $ 38.8357    $& $ 8.44^{+0.60}_{-0.53} $& $10.91^{+0.52}_{-0.47} $& $ 4.79^{+0.10}_{-0.10} $& $22.54^{+0.78}_{-0.78} $ \\
     PLCK\,G$155.3-68.4$  & $0.567    $  & $ 24.3536    $  & $ -8.4557    $& $ 8.01^{+0.46}_{-0.38} $& $10.72^{+0.39}_{-0.36} $& $ 4.20^{+0.06}_{-0.06} $& $18.41^{+0.51}_{-0.51} $ \\
      PLCK\,G$46.2+30.7$  & $0.569    $  & $259.2742    $  & $ 24.0737    $& $ 3.17^{+0.22}_{-0.22} $& $ 3.37^{+0.16}_{-0.15} $& $ 1.26^{+0.04}_{-0.04} $& $ 4.40^{+0.20}_{-0.20} $ \\
     PLCK\,G$239.9-40.0$  & $0.580    $  & $ 71.6966    $  & $-37.0625    $& $ 5.73^{+0.26}_{-0.23} $& $ 7.55^{+0.24}_{-0.23} $& $ 3.36^{+0.04}_{-0.04} $& $13.89^{+0.31}_{-0.31} $ \\
     PLCK\,G$254.6-45.2$  & $0.581    $  & $ 64.3464    $  & $-47.8134    $& $ 4.97^{+0.27}_{-0.27} $& $ 6.45^{+0.24}_{-0.24} $& $ 3.02^{+0.06}_{-0.06} $& $11.69^{+0.40}_{-0.40} $ \\
      RX\,J$0647.7+7015$  & $0.584    $  & $101.9590    $  & $ 70.2481    $& $ 7.78^{+0.21}_{-0.20} $& $10.17^{+0.19}_{-0.19} $& $ 4.80^{+0.04}_{-0.04} $& $22.72^{+0.34}_{-0.34} $ \\
      PLCK\,G$45.3-38.5$  & $0.589    $  & $322.3591    $  & $ -7.6913    $& $ 7.39^{+0.66}_{-0.65} $& $10.49^{+0.66}_{-0.64} $& $ 4.95^{+0.16}_{-0.16} $& $22.33^{+1.18}_{-1.18} $ \\
      PLCK\,G$70.9+49.3$  & $0.602    $  & $239.1098    $  & $ 44.6772    $& $ 5.02^{+0.20}_{-0.21} $& $ 6.47^{+0.18}_{-0.19} $& $ 2.93^{+0.05}_{-0.05} $& $11.71^{+0.31}_{-0.31} $ \\
      PLCK\,G$45.9+57.7$  & $0.609    $  & $229.5866    $  & $ 29.4603    $& $ 5.82^{+0.22}_{-0.22} $& $ 8.82^{+0.23}_{-0.23} $& $ 5.07^{+0.06}_{-0.06} $& $19.56^{+0.35}_{-0.35} $ \\
      PLCK\,G$73.3+67.5$  & $0.609    $  & $215.1709    $  & $ 39.9187    $& $ 6.15^{+0.26}_{-0.25} $& $ 8.77^{+0.26}_{-0.26} $& $ 4.34^{+0.07}_{-0.07} $& $17.97^{+0.47}_{-0.47} $ \\
      PLCK\,G$99.9+58.4$  & $0.615    $  & $213.6952    $  & $ 54.7840    $& $ 7.09^{+0.42}_{-0.42} $& $ 9.98^{+0.39}_{-0.39} $& $ 5.01^{+0.09}_{-0.09} $& $22.03^{+0.79}_{-0.79} $ \\
     PLCK\,G$193.3-46.1$  & $0.620    $  & $ 53.9644    $  & $ -6.9758    $& $ 5.49^{+0.30}_{-0.32} $& $ 7.91^{+0.37}_{-0.41} $& $ 3.25^{+0.04}_{-0.04} $& $12.88^{+0.26}_{-0.26} $ \\
     PLCK\,G$147.3-16.6$  & $0.645    $  & $ 44.1056    $  & $ 40.2885    $& $ 6.51^{+0.29}_{-0.28} $& $ 8.50^{+0.28}_{-0.26} $& $ 4.26^{+0.05}_{-0.05} $& $17.69^{+0.38}_{-0.38} $ \\
     PLCK\,G$260.7-26.3$  & $0.680    $  & $ 94.1429    $  & $-52.4518    $& $ 4.56^{+0.34}_{-0.32} $& $ 5.96^{+0.40}_{-0.36} $& $ 2.86^{+0.06}_{-0.06} $& $10.57^{+0.35}_{-0.35} $ \\
   PSZ2\,G$097.52+51.70$  & $0.700    $  & $223.8379    $  & $ 58.8718    $& $ 4.08^{+0.23}_{-0.23} $& $ 5.77^{+0.26}_{-0.26} $& $ 3.17^{+0.07}_{-0.07} $& $10.63^{+0.39}_{-0.39} $ \\
     PLCK\,G$219.9-34.4$  & $0.700    $  & $ 73.6894    $  & $-20.2851    $& $ 6.77^{+0.33}_{-0.29} $& $ 8.42^{+0.29}_{-0.26} $& $ 4.04^{+0.06}_{-0.06} $& $19.31^{+0.53}_{-0.53} $ \\
   PSZ1\,G$080.66-57.87$  & $0.700    $  & $351.8654    $  & $ -2.0771    $& $ 8.49^{+0.70}_{-0.55} $& $14.69^{+0.74}_{-0.63} $& $10.56^{+0.22}_{-0.22} $& $43.59^{+1.53}_{-1.53} $ \\
     PLCK\,G$208.6-74.4$  & $0.711    $  & $ 30.0695    $  & $-24.9132    $& $ 5.23^{+0.23}_{-0.23} $& $ 7.11^{+0.24}_{-0.23} $& $ 3.83^{+0.06}_{-0.06} $& $15.88^{+0.37}_{-0.37} $ \\
   PSZ1\,G$226.65+28.43$  & $0.724    $  & $134.0858    $  & $  1.7803    $& $ 3.44^{+0.20}_{-0.20} $& $ 4.76^{+0.23}_{-0.22} $& $ 2.55^{+0.04}_{-0.04} $& $ 8.39^{+0.25}_{-0.25} $ \\
   PSZ2\,G$084.10+58.72$  & $0.731    $  & $222.2535    $  & $ 48.5569    $& $ 2.93^{+0.17}_{-0.18} $& $ 3.73^{+0.15}_{-0.16} $& $ 1.84^{+0.03}_{-0.03} $& $ 5.65^{+0.16}_{-0.16} $ \\
   PSZ2\,G$087.39+50.92$  & $0.748    $  & $231.6379    $  & $ 54.1523    $& $ 3.29^{+0.30}_{-0.29} $& $ 4.38^{+0.30}_{-0.28} $& $ 2.41^{+0.07}_{-0.07} $& $ 7.55^{+0.34}_{-0.34} $ \\
   PSZ2\,G$088.98+55.07$  & $0.754    $  & $224.7448    $  & $ 52.8167    $& $ 1.46^{+0.23}_{-0.20} $& $ 1.43^{+0.19}_{-0.17} $& $ 0.54^{+0.03}_{-0.03} $& $ 1.57^{+0.12}_{-0.12} $ \\
   PSZ2\,G$086.93+53.18$  & $0.771    $  & $228.5022    $  & $ 52.8035    $& $ 5.21^{+0.19}_{-0.19} $& $ 7.48^{+0.19}_{-0.18} $& $ 4.63^{+0.06}_{-0.06} $& $17.55^{+0.42}_{-0.42} $ \\
   PLCK\,G$079.95+46.96$  & $0.790    $  & $240.5461    $  & $ 51.0615    $& $ 1.99^{+0.23}_{-0.20} $& $ 2.30^{+0.23}_{-0.20} $& $ 0.98^{+0.03}_{-0.03} $& $ 2.64^{+0.11}_{-0.11} $ \\
     PLCK\,G$352.1-24.00$  & $0.798    $  & $290.2490    $  & $-45.8500    $& $ 5.50^{+0.32}_{-0.31} $& $ 6.79^{+0.36}_{-0.32} $& $ 4.40^{+0.07}_{-0.07} $& $20.12^{+0.51}_{-0.51} $ \\
   PLCK\,G$227.99+38.11$  & $0.810    $  & $143.0891    $  & $  5.6900    $& $ 2.55^{+0.59}_{-0.41} $& $ 2.59^{+0.49}_{-0.37} $& $ 1.15^{+0.07}_{-0.07} $& $ 4.15^{+0.48}_{-0.48} $ \\
       PLCK\,G$091.82+26.11$  & $0.816    $  & $277.7924    $  & $ 62.2429    $& $ 9.83^{+0.52}_{-0.50} $& $14.75^{+0.53}_{-0.48} $& $10.62^{+0.20}_{-0.20} $& $53.33^{+1.87}_{-1.87} $ \\
   PSZ2\,G$208.57-44.31$  & $0.830    $  & $ 60.6477    $  & $-15.6784    $& $ 0.65^{+0.22}_{-0.14} $& $ 0.64^{+0.16}_{-0.12} $& $ 0.35^{+0.04}_{-0.04} $& $ 0.66^{+0.07}_{-0.07} $ \\
   PSZ2\,G$071.82-56.55$  & $0.870    $  & $347.3914    $  & $ -4.1707    $& $ 4.42^{+0.27}_{-0.21} $& $ 6.78^{+0.26}_{-0.23} $& $ 4.96^{+0.09}_{-0.09} $& $17.64^{+0.50}_{-0.50} $ \\
   PSZ2\,G$160.83+81.66$  & $0.890    $  & $186.7420    $  & $ 33.5463    $& $ 5.95^{+0.23}_{-0.22} $& $ 7.53^{+0.21}_{-0.20} $& $ 5.06^{+0.07}_{-0.07} $& $22.03^{+0.49}_{-0.49} $ \\
   PSZ1\,G$254.58-32.16$  & $0.900    $  & $ 83.9566    $  & $-48.0247    $& $ 3.80^{+0.31}_{-0.31} $& $ 4.51^{+0.28}_{-0.29} $& $ 2.38^{+0.06}_{-0.06} $& $ 8.59^{+0.32}_{-0.32} $ \\
    SPT-CL\,J$2146-4633$  & $0.933    $  & $326.6447    $  & $-46.5475    $& $ 3.24^{+0.15}_{-0.16} $& $ 4.76^{+0.17}_{-0.18} $& $ 2.98^{+0.04}_{-0.04} $& $ 9.75^{+0.23}_{-0.23} $ \\
     PLCK\,G$266.6-27.3$  & $0.972    $  & $ 93.9660    $  & $-57.7796    $& $ 8.93^{+0.40}_{-0.40} $& $13.10^{+0.37}_{-0.36} $& $10.27^{+0.18}_{-0.18} $& $54.62^{+1.65}_{-1.65} $ \\
    SPT-CL\,J$2341-5119$  & $1.003    $  & $355.3010    $  & $-51.3286    $& $ 4.17^{+0.21}_{-0.20} $& $ 5.28^{+0.20}_{-0.19} $& $ 3.68^{+0.07}_{-0.07} $& $15.06^{+0.43}_{-0.43} $ \\
    SPT-CL\,J$0546-5345$  & $1.066    $  & $ 86.6551    $  & $-53.7596    $& $ 4.33^{+0.21}_{-0.19} $& $ 5.34^{+0.20}_{-0.19} $& $ 3.67^{+0.05}_{-0.05} $& $15.25^{+0.32}_{-0.32} $ \\
    SPT-CL\,J$2106-5844$  & $1.132    $  & $316.5221    $  & $-58.7421    $& $ 7.01^{+0.49}_{-0.48} $& $ 9.89^{+0.43}_{-0.40} $& $ 9.33^{+0.23}_{-0.23} $& $47.17^{+1.95}_{-1.95} $ \\


==> datatable2.tex <==
&         RXC\,J$2023.0-2056$  & $0.056    $  & $305.7450    $  & $-20.9485    $& $ 1.21^{+0.03}_{-0.03} $& $ 1.03^{+0.02}_{-0.02} $& $ 0.16^{+0.00}_{-0.00} $& $ 0.40^{+0.01}_{-0.01} $ \\
&         RXC\,J$2157.4-0747$  & $0.058    $  & $329.3673    $  & $ -7.8046    $& $ 1.29^{+0.03}_{-0.03} $& $ 1.12^{+0.02}_{-0.02} $& $ 0.15^{+0.00}_{-0.00} $& $ 0.37^{+0.01}_{-0.01} $ \\
&         RXC\,J$0345.7-4112$  & $0.060    $  & $ 56.4428    $  & $-41.2042    $& $ 0.97^{+0.02}_{-0.02} $& $ 0.82^{+0.02}_{-0.02} $& $ 0.15^{+0.00}_{-0.00} $& $ 0.37^{+0.01}_{-0.01} $ \\
&          RXC\,J$0225.1-2928$  & $0.060    $  & $ 36.2877    $  & $-29.4773    $& $ 0.96^{+0.04}_{-0.04} $& $ 0.73^{+0.02}_{-0.02} $& $ 0.12^{+0.00}_{-0.00} $& $ 0.31^{+0.01}_{-0.01} $ \\
&          RXC\,J$1236.7-3354$  & $0.080    $  & $189.1712    $  & $-33.9260    $& $ 1.33^{+0.02}_{-0.02} $& $ 1.21^{+0.02}_{-0.02} $& $ 0.24^{+0.00}_{-0.00} $& $ 0.61^{+0.01}_{-0.01} $ \\
&          RXC\,J$2129.8-5048$ & $0.080    $  & $322.4271    $  & $-50.8167    $& $ 2.26^{+0.06}_{-0.06} $& $ 2.23^{+0.04}_{-0.04} $& $ 0.41^{+0.01}_{-0.01} $& $ 1.19^{+0.02}_{-0.02} $ \\
 PSZ2 G093.92+34.92 &                & $0.081    $  & $258.2029    $  & $ 64.0636    $& $ 5.00^{+0.21}_{-0.15} $& $ 6.00^{+0.19}_{-0.16} $& $ 1.24^{+0.01}_{-0.01} $& $ 4.78^{+0.10}_{-0.10} $ \\
PSZ2\,G222.52+20.58 &         RXC\,J$0821.8+0112$  & $0.082    $  & $125.4614    $  & $  1.1967    $& $ 1.31^{+0.03}_{-0.04} $& $ 1.16^{+0.03}_{-0.03} $& $ 0.22^{+0.00}_{-0.00} $& $ 0.54^{+0.01}_{-0.01} $ \\
PSZ2 G306.77+58.61 &             & $0.084    $  & $194.8438    $  & $ -4.1983    $& $ 4.51^{+0.12}_{-0.11} $& $ 5.63^{+0.13}_{-0.13} $& $ 1.48^{+0.01}_{-0.01} $& $ 5.02^{+0.07}_{-0.07} $ \\
PSZ2 G306.66+61.06 &              & $0.084    $  & $194.6734    $  & $ -1.7622    $& $ 4.21^{+0.05}_{-0.05} $& $ 5.11^{+0.05}_{-0.05} $& $ 1.27^{+0.00}_{-0.00} $& $ 4.25^{+0.03}_{-0.03} $ \\
PSZ2\,G308.64+60.26 &          RXC\,J$1302.8-0230$  & $0.085    $  & $195.7216    $  & $ -2.5170    $& $ 1.89^{+0.03}_{-0.03} $& $ 1.80^{+0.02}_{-0.02} $& $ 0.31^{+0.00}_{-0.00} $& $ 0.83^{+0.01}_{-0.01} $ \\
PSZ2\,G099.57-58.64 &          RXC\,J$0003.8+0203$  & $0.092    $  & $  0.9572    $  & $  2.0657    $& $ 2.11^{+0.04}_{-0.04} $& $ 1.99^{+0.04}_{-0.04} $& $ 0.40^{+0.00}_{-0.00} $& $ 1.15^{+0.01}_{-0.01} $ \\
PSZ2 G321.98-47.96 &             & $0.094    $  & $342.4917    $  & $-64.4294    $& $ 3.73^{+0.06}_{-0.06} $& $ 4.19^{+0.07}_{-0.06} $& $ 1.07^{+0.00}_{-0.00} $& $ 3.51^{+0.03}_{-0.03} $ \\
PSZ2 G336.60-55.43 &             & $0.097    $  & $341.5711    $  & $-52.7261    $& $ 3.99^{+0.08}_{-0.08} $& $ 4.87^{+0.09}_{-0.09} $& $ 1.21^{+0.01}_{-0.01} $& $ 3.95^{+0.04}_{-0.04} $ \\
PSZ2\,G311.62-42.31  &         RXC\,J$2319.6-7313$  & $0.098    $  & $349.9167    $  & $-73.2277    $& $ 1.56^{+0.03}_{-0.03} $& $ 1.74^{+0.03}_{-0.03} $& $ 0.38^{+0.01}_{-0.01} $& $ 0.97^{+0.02}_{-0.01} $ \\
PSZ2\,G332.23-46.37 &          & $0.099    $  & $330.4720    $  & $-59.9454    $& $ 5.64^{+0.09}_{-0.09} $& $ 7.04^{+0.09}_{-0.09} $& $ 1.76^{+0.01}_{-0.01} $& $ 6.61^{+0.06}_{-0.06} $ \\
&          RXC\,J$0211.4-4017$  & $0.101    $  & $ 32.8528    $  & $-40.2915    $& $ 1.00^{+0.02}_{-0.02} $& $ 0.98^{+0.01}_{-0.01} $& $ 0.20^{+0.00}_{-0.00} $& $ 0.48^{+0.01}_{-0.00} $ \\
&          RXC\,J$0049.4-2931$  & $0.108    $  & $ 12.3460    $  & $-29.5206    $& $ 1.62^{+0.04}_{-0.04} $& $ 1.66^{+0.03}_{-0.03} $& $ 0.38^{+0.01}_{-0.01} $& $ 1.00^{+0.02}_{-0.02} $ \\
PSZ2 G053.53+59.52 &              & $0.113    $  & $227.5528    $  & $ 33.5104    $& $ 5.64^{+0.14}_{-0.14} $& $ 7.01^{+0.13}_{-0.13} $& $ 1.71^{+0.01}_{-0.01} $& $ 6.34^{+0.10}_{-0.10} $ \\
PSZ2\,G352.28-77.66   &          RXC\,J$0006.0-3443$  & $0.115    $  & $  1.5015    $  & $-34.7224    $& $ 3.95^{+0.12}_{-0.12} $& $ 4.48^{+0.11}_{-0.11} $& $ 0.97^{+0.01}_{-0.01} $& $ 3.17^{+0.05}_{-0.05} $ \\
PSZ2\,G255.64-25.30   &         RXC\,J$0616.8-4748$  & $0.116    $  & $ 94.2158    $  & $-47.7950    $& $ 2.70^{+0.05}_{-0.05} $& $ 2.86^{+0.04}_{-0.04} $& $ 0.60^{+0.01}_{-0.01} $& $ 1.88^{+0.02}_{-0.02} $ \\
 PSZ2\,G285.52-62.23   &         RXC\,J$0145.0-5300$  & $0.117    $  & $ 26.2433    $  & $-53.0208    $& $ 4.37^{+0.08}_{-0.08} $& $ 4.85^{+0.06}_{-0.06} $& $ 1.08^{+0.01}_{-0.01} $& $ 3.87^{+0.03}_{-0.03} $ \\
&          RXC\,J$1516.3+0005$  & $0.118    $  & $229.0747    $  & $  0.0893    $& $ 3.28^{+0.07}_{-0.04} $& $ 3.61^{+0.04}_{-0.03} $& $ 0.89^{+0.01}_{-0.01} $& $ 2.76^{+0.02}_{-0.02} $ \\
&          RXC\,J$2149.1-3041$  & $0.118    $  & $327.2817    $  & $-30.7013    $& $ 2.25^{+0.03}_{-0.03} $& $ 2.48^{+0.03}_{-0.03} $& $ 0.55^{+0.00}_{-0.00} $& $ 1.58^{+0.02}_{-0.01} $ \\
PSZ2\, G277.38+47.07 &          RXC\,J$1141.4-1216$  & $0.119    $  & $175.3513    $  & $-12.2776    $& $ 2.27^{+0.02}_{-0.02} $& $ 2.45^{+0.02}_{-0.02} $& $ 0.60^{+0.00}_{-0.00} $& $ 1.69^{+0.01}_{-0.01} $ \\
PSZ2\, G000.04+45.13 &          RXC\,J$1516.5-0056$  & $0.120    $  & $229.1842    $  & $ -0.9696    $& $ 2.59^{+0.05}_{-0.04} $& $ 2.99^{+0.04}_{-0.04} $& $ 0.62^{+0.01}_{-0.01} $& $ 1.77^{+0.02}_{-0.02} $ \\
PSZ2\, G256.38+44.04 &          RXC\,J$1044.5-0704$  & $0.134    $  & $161.1370    $  & $ -7.0687    $& $ 2.69^{+0.02}_{-0.02} $& $ 3.32^{+0.04}_{-0.04} $& $ 1.04^{+0.01}_{-0.01} $& $ 2.99^{+0.02}_{-0.02} $ \\
PSZ2 G241.79-24.01 &          RXC\,J$0605.8-3518$  & $0.139    $  & $ 91.4752    $  & $-35.3023    $& $ 3.89^{+0.09}_{-0.09} $& $ 4.66^{+0.08}_{-0.08} $& $ 1.27^{+0.01}_{-0.01} $& $ 4.23^{+0.16}_{-0.03} $ \\
%          R0605\_3518  & $0.139    $  & $ 91.4752    $  & $-35.3023    $& $ 3.87^{+0.06}_{-0.06} $& $ 4.63^{+0.05}_{-0.05} $& $ 1.27^{+0.01}_{-0.01} $& $ 4.23^{+0.04}_{-0.03} $ \\
PSZ2\,G042.81-82.97 &          RXC\,J$0020.7-2542$  & $0.141    $  & $  5.1755    $  & $-25.7080    $& $ 3.84^{+0.06}_{-0.06} $& $ 4.06^{+0.06}_{-0.06} $& $ 1.17^{+0.01}_{-0.01} $& $ 4.05^{+0.04}_{-0.03} $ \\
 PSZ2 G002.77-56.16 &         RXC\,J$2218.6-3853$  & $0.141    $  & $334.6677    $  & $-38.9018    $& $ 4.92^{+0.11}_{-0.11} $& $ 5.67^{+0.07}_{-0.07} $& $ 1.50^{+0.02}_{-0.02} $& $ 5.56^{+0.06}_{-0.06} $ \\
 %         R2218\_3853  & $0.141    $  & $334.6677    $  & $-38.9018    $& $ 4.92^{+0.14}_{-0.14} $& $ 5.66^{+0.11}_{-0.11} $& $ 1.50^{+0.02}_{-0.02} $& $ 5.56^{+0.07}_{-0.06} $ \\
PSZ2 G226.18+76.79 &                & $0.143    $  & $178.8250    $  & $ 23.4049    $& $ 6.24^{+0.06}_{-0.06} $& $ 8.13^{+0.06}_{-0.05} $& $ 2.27^{+0.01}_{-0.01} $& $ 8.84^{+0.06}_{-0.06} $ \\
PSZ2\,G028.77-33.56 &          RXC\,J$2048.1-1750$  & $0.147    $  & $312.0419    $  & $-17.8413    $& $ 4.31^{+0.07}_{-0.07} $& $ 5.50^{+0.05}_{-0.05} $& $ 1.36^{+0.01}_{-0.01} $& $ 4.40^{+0.03}_{-0.03} $ \\
PSZ2 G236.92-26.65 &          RXC\,J$0547.6-3152$  & $0.148    $  & $ 86.9081    $  & $-31.8727    $& $ 5.01^{+0.10}_{-0.10} $& $ 5.97^{+0.08}_{-0.07} $& $ 1.58^{+0.01}_{-0.01} $& $ 5.73^{+0.38}_{-0.04} $ \\
%          R0547\_3152  & $0.148    $  & $ 86.9081    $  & $-31.8727    $& $ 4.98^{+0.09}_{-0.08} $& $ 5.94^{+0.05}_{-0.04} $& $ 1.58^{+0.01}_{-0.01} $& $ 5.73^{+0.04}_{-0.04} $ \\
 PSZ2 G008.47-56.34 &         RXC\,J$2217.7-3543$  & $0.149    $  & $334.4400    $  & $-35.7260    $& $ 3.61^{+0.05}_{-0.05} $& $ 4.37^{+0.04}_{-0.04} $& $ 1.15^{+0.01}_{-0.01} $& $ 3.68^{+0.03}_{-0.03} $ \\
%          R2217\_3543  & $0.149    $  & $334.4400    $  & $-35.7260    $& $ 3.64^{+0.09}_{-0.06} $& $ 4.40^{+0.07}_{-0.06} $& $ 1.15^{+0.01}_{-0.01} $& $ 3.68^{+0.03}_{-0.03} $ \\
PSZ2 G003.93-59.41 &         RXC\,J$2234.5-3744$  & $0.151    $  & $338.6125    $  & $-37.7360    $& $ 7.36^{+0.09}_{-0.09} $& $ 9.87^{+0.10}_{-0.11} $& $ 3.05^{+0.02}_{-0.02} $& $12.28^{+0.12}_{-0.10} $ \\
%         R2234\_3744b  & $0.151    $  & $338.6125    $  & $-37.7360    $& $ 7.31^{+0.14}_{-0.14} $& $ 9.72^{+0.17}_{-0.17} $& $ 3.05^{+0.02}_{-0.02} $& $12.28^{+0.12}_{-0.10} $ \\
 PSZ2 G021.10+33.24 &            & $0.152    $  & $248.1959    $  & $  5.5754    $& $ 8.06^{+0.23}_{-0.22} $& $10.94^{+0.26}_{-0.25} $& $ 2.96^{+0.02}_{-0.02} $& $12.51^{+0.17}_{-0.17} $ \\
PSZ2 G244.71+32.50 & RXC\,J0945.4 -0839  & $0.153    $  & $146.3575    $  & $ -8.6557    $& $ 3.91^{+0.15}_{-0.11} $& $ 5.04^{+0.13}_{-0.10} $& $ 1.43^{+0.02}_{-0.02} $& $ 4.66^{+0.08}_{-0.08} $ \\
 PSZ2\,G018.32-28.50 &         RXC\,J$2014.8-2430$  & $0.154    $  & $303.7154    $  & $-24.5059    $& $ 5.38^{+0.07}_{-0.07} $& $ 7.19^{+0.07}_{-0.07} $& $ 2.08^{+0.02}_{-0.02} $& $ 7.47^{+0.07}_{-0.06} $ \\
PSZ2 G049.22+30.87 &        & $0.164    $  & $260.0417    $  & $ 26.6250    $& $ 5.30^{+0.11}_{-0.11} $& $ 6.97^{+0.12}_{-0.12} $& $ 2.06^{+0.02}_{-0.02} $& $ 7.49^{+0.08}_{-0.08} $ \\
PSZ2 G263.68-22.55 &         RXC\,J$0645.4-5413$  & $0.164    $  & $101.3712    $  & $-54.2273    $& $ 7.38^{+0.18}_{-0.18} $& $10.04^{+0.18}_{-0.18} $& $ 2.81^{+0.02}_{-0.02} $& $11.33^{+0.25}_{-0.08} $ \\
%         R0645\_5413c  & $0.164    $  & $101.3712    $  & $-54.2273    $& $ 7.38^{+0.14}_{-0.14} $& $10.08^{+0.11}_{-0.11} $& $ 2.81^{+0.02}_{-0.02} $& $11.33^{+0.10}_{-0.08} $ \\
PSZ2\, G249.38+33.26 &           RXC\,J$0958.3-1103$  & $0.167    $  & $149.5930    $  & $-11.0644    $& $ 4.17^{+0.22}_{-0.15} $& $ 4.43^{+0.21}_{-0.20} $& $ 1.42^{+0.04}_{-0.04} $& $ 5.21^{+0.15}_{-0.14} $ \\
PSZ2 G097.72+38.12 &               & $0.171    $  & $248.9597    $  & $ 66.2125    $& $ 5.37^{+0.10}_{-0.10} $& $ 7.41^{+0.10}_{-0.10} $& $ 2.20^{+0.01}_{-0.01} $& $ 7.76^{+0.09}_{-0.09} $ \\
PSZ2 G067.17+67.46 &                & $0.171    $  & $216.5105    $  & $ 37.8243    $& $ 8.25^{+0.19}_{-0.19} $& $10.80^{+0.19}_{-0.20} $& $ 3.23^{+0.02}_{-0.02} $& $14.34^{+0.18}_{-0.18} $ \\
 PSZ2 G149.75+34.68 &                & $0.182    $  & $127.7462    $  & $ 65.8398    $& $ 8.07^{+0.53}_{-0.42} $& $11.27^{+0.55}_{-0.45} $& $ 3.04^{+0.06}_{-0.06} $& $13.15^{+0.41}_{-0.41} $ \\
PSZ2 G313.33+61.13 &          RXC\,J$1311.4-0120$  & $0.183    $  & $197.8727    $  & $ -1.3415    $& $ 8.41^{+0.08}_{-0.08} $& $10.69^{+0.06}_{-0.06} $& $ 3.36^{+0.01}_{-0.01} $& $14.93^{+0.08}_{-0.07} $ \\
%           Abell1689  & $0.183    $  & $197.8726    $  & $ -1.3417    $& $ 8.19^{+0.11}_{-0.11} $& $10.79^{+0.10}_{-0.10} $& $ 3.45^{+0.01}_{-0.01} $& $15.24^{+0.12}_{-0.12} $ \\
 PSZ2 G195.75-24.32 &            & $0.203    $  & $ 73.5402    $  & $  2.9212    $& $ 8.31^{+0.22}_{-0.21} $& $11.40^{+0.20}_{-0.18} $& $ 3.46^{+0.03}_{-0.03} $& $14.83^{+0.22}_{-0.22} $ \\
PSZ2 G006.76+30.45 &               A 2163  & $0.203    $  & $243.9399    $  & $ -6.1491    $& $20.10^{+0.61}_{-0.62} $& $32.27^{+0.68}_{-0.70} $& $ 9.50^{+0.08}_{-0.08} $& $55.06^{+1.00}_{-1.00} $ \\
 PSZ2 G182.59+55.83 &         & $0.206    $  & $154.2653    $  & $ 39.0482    $& $ 5.02^{+0.10}_{-0.10} $& $ 6.67^{+0.09}_{-0.09} $& $ 2.15^{+0.02}_{-0.02} $& $ 7.74^{+0.10}_{-0.10} $ \\
 PSZ2 G166.09+43.38 &          & $0.217    $  & $139.4765    $  & $ 51.7315    $& $ 6.61^{+0.14}_{-0.14} $& $ 8.86^{+0.11}_{-0.12} $& $ 2.75^{+0.02}_{-0.02} $& $10.85^{+0.12}_{-0.12} $ \\
PSZ2 G092.71+73.46 &           & $0.223    $  & $203.8298    $  & $ 41.0001    $& $ 7.38^{+0.18}_{-0.18} $& $11.36^{+0.20}_{-0.20} $& $ 3.58^{+0.02}_{-0.02} $& $13.63^{+0.16}_{-0.16} $ \\
 PSZ2\,G055.59+31.85 &          & $0.224    $  & $260.6127    $  & $ 32.1324    $& $ 6.33^{+0.59}_{-0.51} $& $ 9.25^{+0.66}_{-0.58} $& $ 3.15^{+0.13}_{-0.13} $& $12.33^{+0.65}_{-0.65} $ \\
  PSZ2 G072.62+41.46 &            & $0.228    $  & $250.0837    $  & $ 46.7107    $& $11.62^{+0.33}_{-0.24} $& $17.60^{+0.31}_{-0.25} $& $ 6.31^{+0.05}_{-0.05} $& $30.96^{+0.54}_{-0.54} $ \\
 PSZ2 G073.97-27.82 &             & $0.231    $  & $328.4031    $  & $ 17.6949    $& $10.67^{+0.28}_{-0.28} $& $15.86^{+0.32}_{-0.31} $& $ 5.61^{+0.05}_{-0.05} $& $25.89^{+0.38}_{-0.38} $ \\
PSZ2 G294.68-37.01 &               & $0.274    $  & $ 45.9366    $  & $-77.8784    $& $ 7.54^{+0.31}_{-0.32} $& $ 9.76^{+0.26}_{-0.28} $& $ 3.16^{+0.04}_{-0.04} $& $13.35^{+0.28}_{-0.28} $ \\
 PSZ2 G241.76-30.88 &              & $0.275    $  & $ 83.2323    $  & $-37.0270    $& $ 6.40^{+0.23}_{-0.23} $& $ 8.54^{+0.21}_{-0.22} $& $ 2.96^{+0.04}_{-0.04} $& $11.77^{+0.23}_{-0.23} $ \\
PSZ2 G259.98-63.43 &                & $0.284    $  & $ 38.0772    $  & $-44.3464    $& $ 6.99^{+0.21}_{-0.20} $& $10.81^{+0.23}_{-0.23} $& $ 4.34^{+0.04}_{-0.04} $& $16.28^{+0.27}_{-0.27} $ \\
PSZ2 G244.37-32.15 &                 & $0.284    $  & $ 82.2211    $  & $-39.4714    $& $ 6.86^{+0.30}_{-0.33} $& $11.09^{+0.31}_{-0.31} $& $ 4.18^{+0.05}_{-0.05} $& $15.29^{+0.37}_{-0.37} $ \\
PSZ2 G106.87-83.23 &               & $0.292    $  & $ 10.8519    $  & $-20.6229    $& $ 5.91^{+0.25}_{-0.18} $& $ 8.75^{+0.24}_{-0.20} $& $ 3.38^{+0.04}_{-0.04} $& $12.36^{+0.25}_{-0.25} $ \\
PSZ2 G262.27-35.38 &                & $0.295    $  & $ 79.1536    $  & $-54.5090    $& $ 7.81^{+0.81}_{-0.73} $& $11.94^{+0.98}_{-0.96} $& $ 3.90^{+0.17}_{-0.17} $& $15.98^{+0.95}_{-0.95} $ \\
PSZ2 G266.04-21.25 &                & $0.296    $  & $104.6277    $  & $-55.9434    $& $13.92^{+0.29}_{-0.28} $& $20.97^{+0.29}_{-0.28} $& $ 8.72^{+0.06}_{-0.06} $& $46.88^{+0.53}_{-0.53} $ \\
PSZ2 G195.60+44.06 &                & $0.298    $  & $140.1018    $  & $ 30.5028    $& $ 5.36^{+0.09}_{-0.09} $& $ 7.55^{+0.09}_{-0.09} $& $ 2.63^{+0.02}_{-0.02} $& $ 9.46^{+0.11}_{-0.11} $ \\
PSZ2 G125.71+53.86 &               & $0.302    $  & $189.2441    $  & $ 63.1871    $& $ 5.67^{+0.44}_{-0.39} $& $ 7.97^{+0.47}_{-0.43} $& $ 2.99^{+0.09}_{-0.09} $& $11.43^{+0.53}_{-0.53} $ \\
PSZ2 G008.94-81.22 &                & $0.307    $  & $  3.5775    $  & $-30.3863    $& $ 9.81^{+0.24}_{-0.24} $& $16.49^{+0.23}_{-0.22} $& $ 6.70^{+0.05}_{-0.05} $& $27.83^{+0.32}_{-0.32} $ \\
PSZ2 G278.58+39.16 &                & $0.308    $  & $172.9775    $  & $-19.9285    $& $ 8.61^{+0.33}_{-0.30} $& $13.14^{+0.33}_{-0.33} $& $ 4.68^{+0.05}_{-0.05} $& $18.93^{+0.31}_{-0.31} $ \\
PSZ1 G103.58+24.78 &  & $0.330    $  & $286.1007    $  & $ 72.4622    $& $ 4.89^{+0.24}_{-0.23} $& $ 5.34^{+0.21}_{-0.20} $& $ 1.45^{+0.03}_{-0.03} $& $ 6.09^{+0.15}_{-0.15} $ \\
PSZ2 G349.46-59.95 &                  & $0.347    $  & $342.1824    $  & $-44.5305    $& $12.66^{+0.27}_{-0.27} $& $19.02^{+0.27}_{-0.26} $& $ 8.49^{+0.06}_{-0.06} $& $44.19^{+0.63}_{-0.63} $ \\
PSZ2 G083.29-31.03 &                   & $0.412    $  & $337.1405    $  & $ 20.6204    $& $ 8.70^{+0.28}_{-0.28} $& $13.21^{+0.27}_{-0.27} $& $ 5.24^{+0.05}_{-0.05} $& $23.01^{+0.43}_{-0.43} $ \\
PSZ2 G284.41+52.45 &                   & $0.441    $  & $181.5521    $  & $ -8.8002    $& $10.76^{+0.30}_{-0.30} $& $15.71^{+0.28}_{-0.28} $& $ 6.79^{+0.06}_{-0.06} $& $33.82^{+0.65}_{-0.65} $ \\
PSZ2 G056.93-55.08 &                    & $0.444    $  & $340.8387    $  & $ -9.5947    $& $ 9.10^{+0.12}_{-0.12} $& $14.71^{+0.13}_{-0.13} $& $ 7.30^{+0.03}_{-0.03} $& $31.65^{+0.26}_{-0.26} $ \\
PSZ2\, G254.08-58.45 &                   & $0.458    $  & $ 46.0705    $  & $-44.0257    $& $ 5.84^{+0.33}_{-0.33} $& $ 8.21^{+0.33}_{-0.32} $& $ 3.19^{+0.06}_{-0.06} $& $11.74^{+0.32}_{-0.32} $ \\
PSZ2 G265.10-59.50 &                     & $0.500    $  & $ 40.9129    $  & $-48.5611    $& $ 6.13^{+0.63}_{-0.45} $& $ 8.11^{+0.52}_{-0.41} $& $ 3.10^{+0.08}_{-0.08} $& $12.46^{+0.57}_{-0.57} $ \\
PSZ2 G044.77-51.30 &                     & $0.503    $  & $333.7383    $  & $-14.0045    $& $ 7.95^{+0.44}_{-0.43} $& $11.64^{+0.46}_{-0.45} $& $ 5.29^{+0.08}_{-0.08} $& $22.64^{+0.66}_{-0.66} $ \\
PSZ2 G211.21+38.66 &                     & $0.505    $  & $137.7970    $  & $ 17.7760    $& $ 5.48^{+0.22}_{-0.22} $& $ 7.35^{+0.21}_{-0.21} $& $ 3.03^{+0.04}_{-0.04} $& $11.51^{+0.26}_{-0.26} $ \\
 PSZ2 G004.45-19.55 &                      & $0.516    $  & $289.2692    $  & $-33.5228    $& $ 8.73^{+0.48}_{-0.48} $& $12.58^{+0.53}_{-0.52} $& $ 6.28^{+0.15}_{-0.15} $& $28.93^{+1.05}_{-1.05} $ \\
PSZ2 G110.28-87.48 &                        & $0.520    $  & $ 12.2939    $  & $-24.6792    $& $ 4.83^{+0.46}_{-0.36} $& $ 5.45^{+0.43}_{-0.36} $& $ 2.30^{+0.08}_{-0.08} $& $ 8.25^{+0.38}_{-0.38} $ \\
PSZ2 G212.44+63.19 &                       & $0.529    $  & $163.2159    $  & $ 24.2584    $& $ 4.15^{+0.23}_{-0.23} $& $ 5.35^{+0.21}_{-0.21} $& $ 1.93^{+0.04}_{-0.04} $& $ 7.08^{+0.25}_{-0.25} $ \\
PSZ2 G201.50-27.31 &                         & $0.538    $  & $ 73.5471    $  & $ -3.0162    $& $ 7.90^{+0.30}_{-0.29} $& $11.18^{+0.31}_{-0.29} $& $ 6.47^{+0.07}_{-0.07} $& $28.31^{+0.57}_{-0.57} $ \\
PSZ2 G094.56+51.03 &                        & $0.539    $  & $227.0821    $  & $ 57.9164    $& $ 6.15^{+0.25}_{-0.24} $& $ 8.90^{+0.23}_{-0.22} $& $ 3.87^{+0.05}_{-0.05} $& $14.86^{+0.34}_{-0.34} $ \\
PSZ2 G228.16+75.20 &                        & $0.544    $  & $177.3976    $  & $ 22.4011    $& $ 9.36^{+0.64}_{-0.62} $& $14.77^{+0.77}_{-0.73} $& $ 7.08^{+0.17}_{-0.17} $& $31.46^{+1.15}_{-1.15} $ \\
PSZ2 G180.25+21.03 &                         & $0.546    $  & $109.3800    $  & $ 37.7587    $& $12.83^{+0.17}_{-0.17} $& $22.16^{+0.20}_{-0.20} $& $11.41^{+0.04}_{-0.04} $& $56.07^{+0.41}_{-0.41} $ \\
 PSZ2 G111.61-45.71 &                           & $0.546    $  & $  4.6399    $  & $ 16.4362    $& $ 9.21^{+0.24}_{-0.24} $& $14.41^{+0.25}_{-0.25} $& $ 7.49^{+0.07}_{-0.07} $& $34.24^{+0.52}_{-0.52} $ \\
PSZ2 G183.90+42.99 &                           & $0.559    $  & $137.7032    $  & $ 38.8357    $& $ 8.44^{+0.60}_{-0.53} $& $10.91^{+0.52}_{-0.47} $& $ 4.79^{+0.10}_{-0.10} $& $22.54^{+0.78}_{-0.78} $ \\
PSZ2 G155.27-68.42 &                             & $0.567    $  & $ 24.3536    $  & $ -8.4557    $& $ 8.01^{+0.46}_{-0.38} $& $10.72^{+0.39}_{-0.36} $& $ 4.20^{+0.06}_{-0.06} $& $18.41^{+0.51}_{-0.51} $ \\
PSZ2 G046.13+30.72 &                             & $0.569    $  & $259.2742    $  & $ 24.0737    $& $ 3.17^{+0.22}_{-0.22} $& $ 3.37^{+0.16}_{-0.15} $& $ 1.26^{+0.04}_{-0.04} $& $ 4.40^{+0.20}_{-0.20} $ \\
PSZ2 G239.93-39.97 &                               & $0.580    $  & $ 71.6966    $  & $-37.0625    $& $ 5.73^{+0.26}_{-0.23} $& $ 7.55^{+0.24}_{-0.23} $& $ 3.36^{+0.04}_{-0.04} $& $13.89^{+0.31}_{-0.31} $ \\
 PSZ2 G254.64-45.20 &                              & $0.581    $  & $ 64.3464    $  & $-47.8134    $& $ 4.97^{+0.27}_{-0.27} $& $ 6.45^{+0.24}_{-0.24} $& $ 3.02^{+0.06}_{-0.06} $& $11.69^{+0.40}_{-0.40} $ \\
PSZ2 G144.83+25.11 &                               & $0.584    $  & $101.9590    $  & $ 70.2481    $& $ 7.78^{+0.21}_{-0.20} $& $10.17^{+0.19}_{-0.19} $& $ 4.80^{+0.04}_{-0.04} $& $22.72^{+0.34}_{-0.34} $ \\
 PSZ2 G045.32-38.46 &                               & $0.589    $  & $322.3591    $  & $ -7.6913    $& $ 7.39^{+0.66}_{-0.65} $& $10.49^{+0.66}_{-0.64} $& $ 4.95^{+0.16}_{-0.16} $& $22.33^{+1.18}_{-1.18} $ \\
PSZ2 G070.89+49.26 &                               &  $0.602    $  & $239.1098    $  & $ 44.6772    $& $ 5.02^{+0.20}_{-0.21} $& $ 6.47^{+0.18}_{-0.19} $& $ 2.93^{+0.05}_{-0.05} $& $11.71^{+0.31}_{-0.31} $ \\
PSZ2 G045.87+57.70 &                                & $0.609    $  & $229.5866    $  & $ 29.4603    $& $ 5.82^{+0.22}_{-0.22} $& $ 8.82^{+0.23}_{-0.23} $& $ 5.07^{+0.06}_{-0.06} $& $19.56^{+0.35}_{-0.35} $ \\
PSZ2 G073.31+67.52 &                                & $0.609    $  & $215.1709    $  & $ 39.9187    $& $ 6.15^{+0.26}_{-0.25} $& $ 8.77^{+0.26}_{-0.26} $& $ 4.34^{+0.07}_{-0.07} $& $17.97^{+0.47}_{-0.47} $ \\
PSZ2 G099.86+58.45 &                                & $0.615    $  & $213.6952    $  & $ 54.7840    $& $ 7.09^{+0.42}_{-0.42} $& $ 9.98^{+0.39}_{-0.39} $& $ 5.01^{+0.09}_{-0.09} $& $22.03^{+0.79}_{-0.79} $ \\
 PSZ2 G193.31-46.13 &                                & $0.620    $  & $ 53.9644    $  & $ -6.9758    $& $ 5.49^{+0.30}_{-0.32} $& $ 7.91^{+0.37}_{-0.41} $& $ 3.25^{+0.04}_{-0.04} $& $12.88^{+0.26}_{-0.26} $ \\
PLCK\,G147.32-16.59   &                              & $0.645    $  & $ 44.1056    $  & $ 40.2885    $& $ 6.51^{+0.29}_{-0.28} $& $ 8.50^{+0.28}_{-0.26} $& $ 4.26^{+0.05}_{-0.05} $& $17.69^{+0.38}_{-0.38} $ \\
     PLCK\,G$260.7-26.3$  &                         & $0.680    $  & $ 94.1429    $  & $-52.4518    $& $ 4.56^{+0.34}_{-0.32} $& $ 5.96^{+0.40}_{-0.36} $& $ 2.86^{+0.06}_{-0.06} $& $10.57^{+0.35}_{-0.35} $ \\
   PSZ2\,G$097.52+51.70$  &                        &$0.700    $  & $223.8379    $  & $ 58.8718    $& $ 4.08^{+0.23}_{-0.23} $& $ 5.77^{+0.26}_{-0.26} $& $ 3.17^{+0.07}_{-0.07} $& $10.63^{+0.39}_{-0.39} $ \\
PSZ2\,G219.89-34.39 &                              &  $0.700    $  & $ 73.6894    $  & $-20.2851    $& $ 6.77^{+0.33}_{-0.29} $& $ 8.42^{+0.29}_{-0.26} $& $ 4.04^{+0.06}_{-0.06} $& $19.31^{+0.53}_{-0.53} $ \\
   PSZ1\,G$080.66-57.87$  &                      &$0.700    $  & $351.8654    $  & $ -2.0771    $& $ 8.49^{+0.70}_{-0.55} $& $14.69^{+0.74}_{-0.63} $& $10.56^{+0.22}_{-0.22} $& $43.59^{+1.53}_{-1.53} $ \\
PSZ2 G208.61-74.39 &                             & $0.711    $  & $ 30.0695    $  & $-24.9132    $& $ 5.23^{+0.23}_{-0.23} $& $ 7.11^{+0.24}_{-0.23} $& $ 3.83^{+0.06}_{-0.06} $& $15.88^{+0.37}_{-0.37} $ \\
   PSZ1\,G$226.65+28.43$  &                   & $0.724    $  & $134.0858    $  & $  1.7803    $& $ 3.44^{+0.20}_{-0.20} $& $ 4.76^{+0.23}_{-0.22} $& $ 2.55^{+0.04}_{-0.04} $& $ 8.39^{+0.25}_{-0.25} $ \\
   PSZ2\,G$084.10+58.72$  &                   & $0.731    $  & $222.2535    $  & $ 48.5569    $& $ 2.93^{+0.17}_{-0.18} $& $ 3.73^{+0.15}_{-0.16} $& $ 1.84^{+0.03}_{-0.03} $& $ 5.65^{+0.16}_{-0.16} $ \\
   PSZ2\,G$087.39+50.92$  &                   & $0.748    $  & $231.6379    $  & $ 54.1523    $& $ 3.29^{+0.30}_{-0.29} $& $ 4.38^{+0.30}_{-0.28} $& $ 2.41^{+0.07}_{-0.07} $& $ 7.55^{+0.34}_{-0.34} $ \\
   PSZ2\,G$088.98+55.07$  &                   & $0.754    $  & $224.7448    $  & $ 52.8167    $& $ 1.46^{+0.23}_{-0.20} $& $ 1.43^{+0.19}_{-0.17} $& $ 0.54^{+0.03}_{-0.03} $& $ 1.57^{+0.12}_{-0.12} $ \\
   PSZ2\,G$086.93+53.18$  &                   & $0.771    $  & $228.5022    $  & $ 52.8035    $& $ 5.21^{+0.19}_{-0.19} $& $ 7.48^{+0.19}_{-0.18} $& $ 4.63^{+0.06}_{-0.06} $& $17.55^{+0.42}_{-0.42} $ \\
   PLCK\,G$079.95+46.96$  &                   & $0.790    $  & $240.5461    $  & $ 51.0615    $& $ 1.99^{+0.23}_{-0.20} $& $ 2.30^{+0.23}_{-0.20} $& $ 0.98^{+0.03}_{-0.03} $& $ 2.64^{+0.11}_{-0.11} $ \\
PSZ2 G352.05-24.01 &                              & $0.798    $  & $290.2490    $  & $-45.8500    $& $ 5.50^{+0.32}_{-0.31} $& $ 6.79^{+0.36}_{-0.32} $& $ 4.40^{+0.07}_{-0.07} $& $20.12^{+0.51}_{-0.51} $ \\
   PLCK\,G$227.99+38.11$  &                     & $0.810    $  & $143.0891    $  & $  5.6900    $& $ 2.55^{+0.59}_{-0.41} $& $ 2.59^{+0.49}_{-0.37} $& $ 1.15^{+0.07}_{-0.07} $& $ 4.15^{+0.48}_{-0.48} $ \\
PSZ2\,G091.83+26.11 &                               & $0.816    $  & $277.7924    $  & $ 62.2429    $& $ 9.83^{+0.52}_{-0.50} $& $14.75^{+0.53}_{-0.48} $& $10.62^{+0.20}_{-0.20} $& $53.33^{+1.87}_{-1.87} $ \\
   PSZ2\,G$208.57-44.31$  &                        & $0.830    $  & $ 60.6477    $  & $-15.6784    $& $ 0.65^{+0.22}_{-0.14} $& $ 0.64^{+0.16}_{-0.12} $& $ 0.35^{+0.04}_{-0.04} $& $ 0.66^{+0.07}_{-0.07} $ \\
   PSZ2\,G$071.82-56.55$  &                          & $0.870    $  & $347.3914    $  & $ -4.1707    $& $ 4.42^{+0.27}_{-0.21} $& $ 6.78^{+0.26}_{-0.23} $& $ 4.96^{+0.09}_{-0.09} $& $17.64^{+0.50}_{-0.50} $ \\
   PSZ2\,G$160.83+81.66$  &                         & $0.890    $  & $186.7420    $  & $ 33.5463    $& $ 5.95^{+0.23}_{-0.22} $& $ 7.53^{+0.21}_{-0.20} $& $ 5.06^{+0.07}_{-0.07} $& $22.03^{+0.49}_{-0.49} $ \\
   PSZ1\,G$254.58-32.16$  &                          & $0.900    $  & $ 83.9566    $  & $-48.0247    $& $ 3.80^{+0.31}_{-0.31} $& $ 4.51^{+0.28}_{-0.29} $& $ 2.38^{+0.06}_{-0.06} $& $ 8.59^{+0.32}_{-0.32} $ \\
    SPT-CL\,J$2146-4633$  &                           & $0.933    $  & $326.6447    $  & $-46.5475    $& $ 3.24^{+0.15}_{-0.16} $& $ 4.76^{+0.17}_{-0.18} $& $ 2.98^{+0.04}_{-0.04} $& $ 9.75^{+0.23}_{-0.23} $ \\
     PLCK\,G$266.6-27.3$  &                            & $0.972    $  & $ 93.9660    $  & $-57.7796    $& $ 8.93^{+0.40}_{-0.40} $& $13.10^{+0.37}_{-0.36} $& $10.27^{+0.18}_{-0.18} $& $54.62^{+1.65}_{-1.65} $ \\
    SPT-CL\,J$2341-5119$  &                           & $1.003    $  & $355.3010    $  & $-51.3286    $& $ 4.17^{+0.21}_{-0.20} $& $ 5.28^{+0.20}_{-0.19} $& $ 3.68^{+0.07}_{-0.07} $& $15.06^{+0.43}_{-0.43} $ \\
    SPT-CL\,J$0546-5345$  &                           & $1.066    $  & $ 86.6551    $  & $-53.7596    $& $ 4.33^{+0.21}_{-0.19} $& $ 5.34^{+0.20}_{-0.19} $& $ 3.67^{+0.05}_{-0.05} $& $15.25^{+0.32}_{-0.32} $ \\
    SPT-CL\,J$2106-5844$  &                            & $1.132    $  & $316.5221    $  & $-58.7421    $& $ 7.01^{+0.49}_{-0.48} $& $ 9.89^{+0.43}_{-0.40} $& $ 9.33^{+0.23}_{-0.23} $& $47.17^{+1.95}_{-1.95} $ \\

